Automatic Error Analysis for Document-level Information Extraction

Document-level information extraction (IE) tasks have recently begun to be revisited in earnest using the end-to-end neural network techniques that have been successful on their sentence-level IE counterparts. Evaluation of the approaches, however, has been limited in a number of dimensions. In particular, the precision/recall/F1 scores typically reported provide few insights on the range of errors the models make. We build on the work of Kummerfeld and Klein (2013) to propose a transformation-based framework for automating error analysis in document-level event and (N-ary) relation extraction. We employ our framework to compare two state-of-the-art document-level template-filling approaches on datasets from three domains; and then, to gauge progress in IE since its inception 30 years ago, vs. four systems from the MUC-4 (1992) evaluation.

==> acl2021/tables/data_stats_2.tex <==
\begin{table*}[t]
\small \centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c}
\toprule
      & \begin{tabular}[c]{@{}l@{}}\# docs \\ (train/val/test/unannot.)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# tokens per doc \\ (min/max/avg.)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# templates per \\ relevant doc (max/avg.)\end{tabular} & 
      \begin{tabular}[c]{@{}l@{}}\% docs with \\ 0 templates \end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}- MUC-4 \\ \cite{muc-1992-message}\end{tabular}    &    1300 / 200 / 200 / 0                             &              31 / 1695 / 362                        &  14 / 1.61 & 44.59 \\
- ProMED\footnote{http://www.promedmail.org} &     125 / 12 / 108 / 4979                           &        57 / 4417 / 621                            &  9 / 1.55   &   19.83 \\
\begin{tabular}[c]{@{}l@{}}- SciREX \\ \cite{jain-etal-2020-scirex}\end{tabular}    &     304 / 66 / 66 / 0                            &    1153 / 13155 / 5401                                   &     16 / 2.28  & 0.00  \\ \bottomrule
\end{tabular}
% }
\caption{Dataset Statistics. A relevant document has one or more templates.}
\label{tab:stats2}
\end{table*}

==> acl2021/tables/f1data.tex <==
\begin{table}[!t]
\small \centering
\begin{tabular}{l|ccc}
\toprule
               & SciREX & ProMED & MUC-4 \\ \midrule
DyGIE++ (BERT) &  22.47\%     &  35.01\%      &    45.79\%   \\
DyGIE++ (SciBERT) &  25.39\%     &  38.15\%      &    -  \\
GTT (BERT)     &  21.54\%      &   {\bf 44.64}\%     &    {\bf 49.00\%}   \\
GTT (SciBERT)  &  {\bf 27.68}\%      &   42.96\%    &   -   \\ \bottomrule
\end{tabular}
\caption{F1 Scores for the Neural Models on SciREX, ProMED, and MUC-4}
\label{tab:f1}
\end{table}

==> acl2021/tables/model_metric_results.tex <==
\begin{table}[h]
\small \centering
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
\multicolumn{1}{c|}{Models} & SciREX & ProMED & MUC-4 \\ \midrule
DyGIE++ (BERT) & 27.85 / 18.83 / 22.47
 & 51.13 / 26.62 / 35.01 & 61.90 / 36.33 / 45.79 \\
DyGIE++ (SciBERT) & 30.47 / 21.76 / 25.39 & 52.55 / 29.94 / 38.15 & - \\
GTT (BERT) & 52.86 / 13.53 / 21.54 & 68.58 / 33.09 / {\bf 44.64} & 63.18 / 40.02 / {\bf 49.00} \\
GTT (SciBERT) & 53.68 / 18.65 / {\bf 27.68} & 64.68 / 32.16 / 42.96 & - \\ 
\bottomrule
\end{tabular}
% }
\caption{Precision, Recall and F1 Scores (\%).}
% \vspace{-0.5cm}
\label{tab:modelstats}
\end{table}

==> acl2021/tables/progress_muc.tex <==
\begin{table}[!t]
\small \centering
\begin{tabular}{l|ccc}
\toprule
               & Precision & Recall & F1 \\ \midrule
GE NLToolset &  56.69\%     &  {\bf 52.09\%}      &    {\bf54.29\%}   \\
NYU PROTEUS     &  34.23\%      &   31.28\%     &    32.69\%   \\
SRI FASTUS  &  48.47\%      &   38.42\%    &   42.86\%   \\ 
UMass CIRCUS  &  48.62\%      &   39.04\%    &   43.30\%  \\
\midrule
GTT (BERT) & {\bf 63.18}\% & 40.02\% & 49.00\% \\
DyGIE++ (BERT) & 61.90\% & 36.33\% & 45.79\%\\
\bottomrule
\end{tabular}
\caption{Precision, Recall, and F1 scores for models on the MUC-4 dataset. The first four models were developed in 1992, while the last two models are recent and use neural-based methods.}
\label{tab:progressmuc}
\end{table}

==> acl2021/tables/progress_span.tex <==
\begin{table}[!t]
\small \centering
\begin{tabular}{c|c}
\toprule
               Predicted & Gold Match \\ \midrule
\parbox[t]{0.2\textwidth}{power lines {\bf along the road}} & \parbox[t]{0.2\textwidth}{power lines}   \\ & \\
\parbox[t]{0.2\textwidth}{enrique ruiz{\bf, retired}} & \parbox[t]{0.2\textwidth}{enrique ruiz}  \\ & \\
\parbox[t]{0.2\textwidth}{{\bf maoist} shining path group} & \parbox[t]{0.2\textwidth}{shining path}  \\ & \\
 \parbox[t]{0.2\textwidth}{
group of unidentified individuals {\bf who hurled a bomb ... passing vehicle}} & \parbox[t]{0.2\textwidth}{group of unidentified individuals}  \\ & \\
%\hline
%\parbox[t]{0.2\textwidth}{his students} & \parbox[t]{0.2\textwidth}{{\bf four terrorists who claimed to be} his students}  \\ & \\
%\parbox[t]{0.2\textwidth}{urban command} & \parbox[t]{0.2\textwidth}{{\bf manuel jose arce} urban command}  \\ & \\
%\parbox[t]{0.2\textwidth}{alleged terrorists} & \parbox[t]{0.2\textwidth}{{\bf four} alleged terrorists}  \\ & \\
%\parbox[t]{0.2\textwidth}{luis} & \parbox[t]{0.2\textwidth}{luis {\bf carlos galan}}  \\ & \\
%\parbox[t]{0.2\textwidth}{mejia rodriguez} & \parbox[t]{0.2\textwidth}{{\bf rosalio} mejia rodriguez}  \\ & \\
\bottomrule
\end{tabular}
\caption{Span Errors in early models. The differences between the predicted mention and its best gold mention match according to our analysis tool are in bold.}
\label{tab:progressspan}
\end{table}
               

==> acl2021/tables/promed_example_err_type.tex <==
\begin{table*}[h]
\centering
\small
% \resizebox{0.9\textwidth}{0.8\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{|p{0.05\textwidth}|p{0.2\textwidth}|p{0.2\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|}
\hline
\multicolumn{1}{|c|}{} &
\multicolumn{1}{c|}{{\bf Error Types}}                         & \multicolumn{1}{c|}{{\bf Transformations(s)}}                              & \multicolumn{1}{c|}{{\bf Predicted}} & \multicolumn{1}{c|}{{\bf Gold}} \\ \hline
i) & Span Error & Alter Span & Victims: {\bf[\color{black}young fattening cattle]} & Victims: [young fattening cattle and sheep] \\ \hline
ii) & Duplicate Role Filler & Remove Duplicate Role Filler & Disease: [west nile fever], {\bf [\color{black}west nile virus]} & Disease: [west nile fever, west nile virus] \\ \hline
iii) & Within Template Incorrect Role & Alter Role & \parbox[t]{0.2\textwidth}{{\bf \color{torange} T1:} \\ Disease: {\bf [\color{black} 2 humans]} \\ Victims: ---} & \parbox[t]{0.2\textwidth}{{\bf \color{torange} T1:} \\ Disease: --- \\ Victims: [2 humans]} \\ \hline
iv) & Wrong Template For Role Filler & Remove Cross Template Spurious Role Filler & \parbox[t]{0.2\textwidth}{{ \bf \color{torange} T1:} \\ Country: [netherlands] \\ Victims: {\bf \color{black} [770 cases]}} &  \parbox[t]{0.2\textwidth}{{\bf \color{torange} T1:} \\ Country: [netherlands] \\ Victims: [its 11th case]} \\ 
& & & & \parbox[t]{0.2\textwidth}{{\bf \color{tpurple} T2:} \\ Country: [united kingdom] \\ Victims: [770 cases] } \\
\hline
v) & Spurious Template & Remove Spurious Template & \parbox[t]{0.2\textwidth}{{\bf \color{black}T1: Country: [china] }} & \multicolumn{1}{c|}{---} \\ \hline
vi) & Missing Template & Introduce Missing Template &  \multicolumn{1}{c|}{{\bf \color{black}---}} & \parbox[t]{0.2\textwidth}{{\bf \color{torange} T1}: \\ Country: [germany] \\Disease: [fmd] \\ Victims: [2 pigs]} \\ \hline
\end{tabular}}
\caption{Some examples of the Error Types taken from the ProMED dataset. For each template, in every role, the role fillers within brackets refer to the same entity, while role fillers in different brackets refer to different entities. The text in bold black indicates the error in the prediction.}
\label{tab:errexpromed}
\end{table*}

==> old-intro.tex <==
\section{Introduction}
\label{sec:intro}



Information extraction research has
almost uniformly focused on \textit{sentence-level} domain- or task-specific relation and event extraction \cite{grishman2019twenty}.   
These information extraction approaches involve identifying lexical {\it triggers} or {\it predicates} \textemdash words or phrases that indicate the occurrence of a relation or event as well as {\it arguments} \textemdash entities that fill specific roles in the relation/event, followed by assigning arguments to the correct trigger. 

Both feature-based and neural methods have been proposed for this task. For example, \cite{surdeanu-etal-2003-using} \bw{no parenthesis here} uses inductive decision tree learning with features obtained from parsing and named entity recognition to automatically identify predicate argument structures for information extraction while \cite{li-etal-2013-joint} uses a structured perceptron with token-based decoder to jointly predict event triggers and arguments using global features such as context and dependency paths between two triggers. \bw{Last sentence is 10-line long} DyGIE++ \cite{wadden-etal-2019-entity} enumerates candidate text spans (arguments) and encodes them using BERT, a contextual language model to get span representations, which are then refined by propagating updates from a graph representing relations between event triggers and their arguments. 

Unfortunately, all these methods require the lexical trigger of the relation or event to occur in the same sentence as the associated
arguments to be extracted, which makes them unsuitable when information corresponding to a particular relation or event is spread across multiple sentences, or even paragraphs \textemdash as the entire discourse context of the document must now be understood in order to be interpret text correctly.

For example, in Figure \ref{fig:task}, a sentence-level approach should be able to identify "close to half a million Honduran chickens" as the {\sc Victim} because it is in the same sentence as the trigger expression "the disease has killed", but it would miss "Newcastle" as the associated {\sc Disease}, as it was mentioned in the previous paragraph.


In addition, for easy interpretation of the output by end-users, it is important that distinct mentions of the same relation, event, or argument in different sentences are recognized as co-referent, so as to avoid the extraction of duplicates.

As a result, we argue that more focus should be put on the problem of \textit{document-level} information extraction (IE). \cc{in which ... [formal description of the problem...or is it too early? probably too early.]} %
Though recently there have been works focusing on building modern NLP models for the document level IE task ~\cite{du-etal-2021-template, li-etal-2021-document, jain-etal-2020-scirex}, %
there has not been a systematic investigation and analysis on models' error types across several document-level extraction datasets from different domains.

\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{
\includegraphics{./figures/error_analysis_eg.pdf}
}
\caption{The document-level extraction task (left) and the automatic error analysis process (right). Our system performs a set of transformations on the predicted templates to convert them into the corresponding gold standard templates. Transformation steps are mapped to corresponding error types to produce informative error statistics.}
\label{fig:task}
\end{figure*}

In this work, we first provide an abstraction of the problem setting (Section~\ref{sec:taskdef}), and present a comparison between several representative document-level IE datasets.
Then, inspired by the work of \newcite{kummerfeld-klein-2013-error} on tackling the error analysis challenge for co-reference resolution, we introduce a framework for automating the process of error analysis for document-level information extraction / template filling. Our framework automatically changes the predicted outputs into their gold standard counterparts through a set of transformations (Figure~\ref{fig:transformation}), then it maps each step of transformation into sensible and linguistically motivated error types (Table~\ref{tab:errex}). \xd{(to add more)}

Next, we apply two state-of-the-art neural template filling methods to two document-level information extraction tasks from multiple domains including scientific literature. %
We analyze their behaviors and errors in their predictions via our automatic framework.

We also retrieve predictions for four systems on the MUC-4 \cite{muc-1992-message} dataset: the GE NLToolset \cite{krupka-etal-1992-ge}, New York University's PROTEUS 
 \cite{grishman-etal-1992-new-york}, SRI International's FASTUS \cite{hobbs-etal-1992-sri} and University of Massachusetts's CIRCUS  \cite{lehnert-etal-1992-university-massachusetts}. We analyze errors in their output using our automatic framework to measure progress in information extraction and compare the performance of early systems versus machine learning/deep learning systems used currently.

\cc{summarize findings.}












==> tables/error_trans_desc.tex <==
% error-trans description table
% \begin{table*}[t]
% \begin{tabular}{|l|c|c|c|}
% \toprule
%       & \begin{tabular}[c]{@{}l@{}} Error Types \end{tabular} & \begin{tabular}[c]{@{}l@{}} Transformation(s) \end{tabular} & \begin{tabular}[c]{@{}l@{}} Description \end{tabular} \\ \midrule
%       i) & Span Error & Alter Span & Exact match to the role filler upon \\
%       & & & span alteration. \\
%       \hline
%       ii) & Duplicate Role Filler & Remove Duplicate & Spurious Role Filler which is co-referent \\
%       & (Spurious) & Role Filler & to an already matched role-filler and \\
%       & & & treated as a separate entity. \\
%       & & & (coreference resolution error) \\
%       \hline
%       iii) & Duplicate Partially & Alter Span & Spurious Role Filler which is co-referent \\
%       & Matched Role Filler & + Remove Duplicate & to an already matched role-filler upon \\
%       & (Spurious) & Role Filler & span alteration and treated \\ 
%       & & & as a separate entity. \\
%       & & & (span extraction error + \\ 
%       & & & coreference resolution error) \\
%       \hline
%       iv) &  & Alter Role  & Spurious Role Filler which is assigned \\
%       & Incorrect Role & & to the incorrect role within the same template \\
%       & & & (role assignment error) \\
%       \hline
%       v) &  & Alter Span & Spurious Role Filler which is assigned \\
%       & Incorrect Role & + Alter Role & to the incorrect role within \\
%       & + Partially Matched & & the same template upon span alteration. \\
%       & Filler & & (span extraction error + role assignment error) \\
%       \hline
%       vi) & Wrong Template & Remove Cross Template & Spurious Role Filler which is \\
%       & for Role Filler & Spurious Role Filler & assigned to the correct role in another template, \\
%       & & & i.e., would be correct if it had \\
%       & & & been placed in another template. \\
%       & & & (event assignment error) \\
%       \hline
%       vii) & Wrong Template & Alter Span  & Spurious Role Filler which is assigned \\
%       & for Partially Matched & + Remove Cross Template & to the correct role in another template \\
%       & Role Filler & Spurious Role Filler & upon span alteration. \\
%       & & & (span extraction error + event assignment error) \\
%       \hline
%       viii) & Wrong Template & Alter Role & Spurious Role Filler which is assigned \\
%       & + Wrong Role & + Remove Cross Template & to another role in another template. \\
%       & (Spurious) & Spurious Role Filler & (event assignment error + role assignment error) \\
%       \hline
%       ix) & Wrong Template & Alter Span & Spurious Role Filler which is \\
%       & + Wrong Role & + Alter Role & assigned to another role in \\
%       & + Partially Matched & + Remove Cross Template & another template upon span alteration. \\
%       & Filler & Spurious Role Filler & (span extraction error \\
%       & & & + event assignment error \\
%       & & & + role assignment error)\\
%       \hline
%       x) & Spurious Role Filler & Remove Role Filler randomly extracted \\
%       & & Spurious Role Filler & from the text with no \\ 
%       & & & connection to the gold templates.\\
%       \hline 
%       xi) & Missing Role Filler & Introduce & Role Filler present in the gold template \\
%       & & Role Filler & but not the predicted template for a given role. \\
%       \hline
%       xii) & Spurious Template & Remove & Extra predicted template that cannot \\
%       & & Spurious Template & be matched to a gold template. \\
%       \hline
%       xiii) & Missing Template & Introduce & Remaining gold template that has \\
%       & & Missing Template & no matching predicted template. \\
% \bottomrule
% \end{tabular}
% \caption{Error Types and their Respective Transformation(s)}
% \label{tab:errtrans}
% \end{table*}
